Mode Collapse of Mean-Field Variational Inference

Mean-field variational inference (MFVI) is a widely used method for approximating high-dimensional probability distributions by product measures. It has been empirically observed that MFVI optimizers often suffer from \emph{mode collapse}. For example, when the target measure $\pi$ is a mixture $\pi = w P_0 + (1 - w) P_1$, the MFVI optimizer tends to place most of its mass near a single component of the mixture. This work provides the first \emph{theoretical} explanation of mode collapse in MFVI. Starting from two-component mixtures, we introduce the notion of \emph{$\varepsilon$-separateness} to quantify the separation of the mixture components. We derive explicit bounds on the mass that any MFVI optimizer assigns to each component, when $P_0$ and $P_1$ are $\varepsilon$-separated for sufficiently small $\varepsilon$. We further extend this analysis to mixture target distributions with multiple components. Our results reveal that the occurrence of mode collapse crucially depends on the relative position of the components. To address this issue, we propose \emph{rotational variational inference (RoVI)}, which augments MFVI with a rotation matrix. The numerical studies support our theoretical findings and illustrate improved mode coverage with RoVI in Bayesian mixture posteriors, including a real-data example.

==> mathsymbols.tex <==
\usepackage{amsfonts,bbm,bm}
%
\RequirePackage[capitalize]{cleveref}

%

%
\newcommand{\Ta}{\mathrm{a}}
\newcommand{\Tb}{\mathrm{b}}
\newcommand{\Tc}{\mathrm{c}}
\newcommand{\Td}{\mathrm{d}}
\newcommand{\Te}{\mathrm{e}}
\newcommand{\Tf}{\mathrm{f}}
\newcommand{\Tg}{\mathrm{g}}
\newcommand{\Th}{\mathrm{h}}
\newcommand{\Ti}{\mathrm{i}}
\newcommand{\Tj}{\mathrm{j}}
\newcommand{\Tk}{\mathrm{k}}
\newcommand{\Tl}{\mathrm{l}}
\newcommand{\Tm}{\mathrm{m}}
\newcommand{\Tn}{\mathrm{n}}
\newcommand{\To}{\mathrm{o}}
\newcommand{\Tp}{\mathrm{p}}
\newcommand{\Tq}{\mathrm{q}}
\newcommand{\Tr}{\mathrm{r}}
\newcommand{\Ts}{\mathrm{s}}
\newcommand{\Tt}{\mathrm{t}}
\newcommand{\Tu}{\mathrm{u}}
\newcommand{\Tv}{\mathrm{v}}
\newcommand{\Tw}{\mathrm{w}}
\newcommand{\Tx}{\mathrm{x}}
\newcommand{\Ty}{\mathrm{y}}
\newcommand{\Tz}{\mathrm{z}}

%
\newcommand{\TA}{\mathrm{A}}
\newcommand{\TB}{\mathrm{B}}
\newcommand{\TC}{\mathrm{C}}
\newcommand{\TD}{\mathrm{D}}
\newcommand{\TE}{\mathrm{E}}
\newcommand{\TF}{\mathrm{F}}
\newcommand{\TG}{\mathrm{G}}
\renewcommand{\TH}{\mathrm{H}}
\newcommand{\TI}{\mathrm{I}}
\newcommand{\TJ}{\mathrm{J}}
\newcommand{\TK}{\mathrm{K}}
\newcommand{\TL}{\mathrm{L}}
\newcommand{\TM}{\mathrm{M}}
\newcommand{\TN}{\mathrm{N}}
\newcommand{\TO}{\mathrm{O}}
\newcommand{\TP}{\mathrm{P}}
\newcommand{\TQ}{\mathrm{Q}}
\newcommand{\TR}{\mathrm{R}}
\newcommand{\TS}{\mathrm{S}}
\newcommand{\TT}{\mathrm{T}}
\newcommand{\TU}{\mathrm{U}}
\newcommand{\TV}{\mathrm{V}}
\newcommand{\TW}{\mathrm{W}}
\newcommand{\TX}{\mathrm{X}}
\newcommand{\TY}{\mathrm{Y}}
\newcommand{\TZ}{\mathrm{Z}}

%
\newcommand{\Ba}{\mathbf{a}}
\newcommand{\Bb}{\mathbf{b}}
\newcommand{\Bc}{\mathbf{c}}
\newcommand{\Bd}{\mathbf{d}}
\newcommand{\Be}{\mathbf{e}}
\newcommand{\Bf}{\mathbf{f}}
\newcommand{\Bg}{\mathbf{g}}
\newcommand{\Bh}{\mathbf{h}}
\newcommand{\Bi}{\mathbf{i}}
\newcommand{\Bj}{\mathbf{j}}
\newcommand{\Bk}{\mathbf{k}}
\newcommand{\Bl}{\mathbf{l}}
\newcommand{\Bm}{\mathbf{m}}
\newcommand{\Bn}{\mathbf{n}}
\newcommand{\Bo}{\mathbf{o}}
\newcommand{\Bp}{\mathbf{p}}
\newcommand{\Bq}{\mathbf{q}}
\newcommand{\Br}{\mathbf{r}}
\newcommand{\Bs}{\mathbf{s}}
\newcommand{\Bt}{\mathbf{t}}
\newcommand{\Bu}{\mathbf{u}}
\newcommand{\Bv}{\mathbf{v}}
\newcommand{\Bw}{\mathbf{w}}
%
\newcommand{\Bx}{\bm{x}}
\newcommand{\By}{\mathbf{y}}
\newcommand{\Bz}{\mathbf{z}}


%
\newcommand{\BA}{\mathbf{A}}
\newcommand{\BB}{\mathbf{B}}
\newcommand{\BC}{\mathbf{C}}
\newcommand{\BD}{\mathbf{D}}
\newcommand{\BE}{\mathbf{E}}
\newcommand{\BF}{\mathbf{F}}
\newcommand{\BG}{\mathbf{G}}
\newcommand{\BH}{\mathbf{H}}
\newcommand{\BI}{\mathbf{I}}
\newcommand{\BJ}{\mathbf{J}}
\newcommand{\BK}{\mathbf{K}}
\newcommand{\BL}{\mathbf{L}}
\newcommand{\BM}{\mathbf{M}}
\newcommand{\BN}{\mathbf{N}}
\newcommand{\BO}{\mathbf{O}}
\newcommand{\BP}{\mathbf{P}}
\newcommand{\BQ}{\mathbf{Q}}
\newcommand{\BR}{\mathbf{R}}
\newcommand{\BS}{\mathbf{S}}
\newcommand{\BT}{\mathbf{T}}
\newcommand{\BU}{\mathbf{U}}
\newcommand{\BV}{\mathbf{V}}
\newcommand{\BW}{\mathbf{W}}
\newcommand{\BX}{\mathbf{X}}
\newcommand{\BY}{\mathbf{Y}}
\newcommand{\BZ}{\mathbf{Z}}

%
\newcommand{\BIa}{{\boldsymbol{a}}}
\newcommand{\BIb}{{\boldsymbol{b}}}
\newcommand{\BIc}{{\boldsymbol{c}}}
\newcommand{\BId}{{\boldsymbol{d}}}
\newcommand{\BIe}{{\boldsymbol{e}}}
\newcommand{\BIf}{{\boldsymbol{f}}}
\newcommand{\BIg}{{\boldsymbol{g}}}
\newcommand{\BIh}{{\boldsymbol{h}}}
\newcommand{\BIi}{{\boldsymbol{i}}}
\newcommand{\BIj}{{\boldsymbol{j}}}
\newcommand{\BIk}{{\boldsymbol{k}}}
\newcommand{\BIl}{{\boldsymbol{l}}}
\newcommand{\BIm}{{\boldsymbol{m}}}
\newcommand{\BIn}{{\boldsymbol{n}}}
\newcommand{\BIo}{{\boldsymbol{o}}}
\newcommand{\BIp}{{\boldsymbol{p}}}
\newcommand{\BIq}{{\boldsymbol{q}}}
\newcommand{\BIr}{{\boldsymbol{r}}}
\newcommand{\BIs}{{\boldsymbol{s}}}
\newcommand{\BIt}{{\boldsymbol{t}}}
\newcommand{\BIu}{{\boldsymbol{u}}}
\newcommand{\BIv}{{\boldsymbol{v}}}
\newcommand{\BIw}{{\boldsymbol{w}}}
\newcommand{\BIx}{{\boldsymbol{x}}}
\newcommand{\BIy}{{\boldsymbol{y}}}
\newcommand{\BIz}{{\boldsymbol{z}}}

%
\newcommand{\BIA}{{\boldsymbol{A}}}
\newcommand{\BIB}{{\boldsymbol{B}}}
\newcommand{\BIC}{{\boldsymbol{C}}}
\newcommand{\BID}{{\boldsymbol{D}}}
\newcommand{\BIE}{{\boldsymbol{E}}}
\newcommand{\BIF}{{\boldsymbol{F}}}
\newcommand{\BIG}{{\boldsymbol{G}}}
\newcommand{\BIH}{{\boldsymbol{H}}}
\newcommand{\BII}{{\boldsymbol{I}}}
\newcommand{\BIJ}{{\boldsymbol{J}}}
\newcommand{\BIK}{{\boldsymbol{K}}}
\newcommand{\BIL}{{\boldsymbol{L}}}
\newcommand{\BIM}{{\boldsymbol{M}}}
\newcommand{\BIN}{{\boldsymbol{N}}}
\newcommand{\BIO}{{\boldsymbol{O}}}
\newcommand{\BIP}{{\boldsymbol{P}}}
\newcommand{\BIQ}{{\boldsymbol{Q}}}
\newcommand{\BIR}{{\boldsymbol{R}}}
\newcommand{\BIS}{{\boldsymbol{S}}}
\newcommand{\BIT}{{\boldsymbol{T}}}
\newcommand{\BIU}{{\boldsymbol{U}}}
\newcommand{\BIV}{{\boldsymbol{V}}}
\newcommand{\BIW}{{\boldsymbol{W}}}
\newcommand{\BIX}{{\boldsymbol{X}}}
\newcommand{\BIY}{{\boldsymbol{Y}}}
\newcommand{\BIZ}{{\boldsymbol{Z}}}

%
\newcommand{\CA}{\mathcal{A}}
\newcommand{\CB}{\mathcal{B}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\CD}{\mathcal{D}}
\newcommand{\CE}{\mathcal{E}}
\newcommand{\CF}{\mathcal{F}}
\newcommand{\CG}{\mathcal{G}}
\newcommand{\CH}{\mathcal{H}}
\newcommand{\CI}{\mathcal{I}}
\newcommand{\CJ}{\mathcal{J}}
\newcommand{\CK}{\mathcal{K}}
\newcommand{\CL}{\mathcal{L}}
\newcommand{\CM}{\mathcal{M}}
\newcommand{\CN}{\mathcal{N}}
\newcommand{\CO}{\mathcal{O}}
\newcommand{\CP}{\mathcal{P}}
\newcommand{\CQ}{\mathcal{Q}}
\newcommand{\CR}{\mathcal{R}}
\newcommand{\CS}{\mathcal{S}}
\newcommand{\CT}{\mathcal{T}}
\newcommand{\CU}{\mathcal{U}}
\newcommand{\CV}{\mathcal{V}}
\newcommand{\CW}{\mathcal{W}}
\newcommand{\CX}{\mathcal{X}}
\newcommand{\CY}{\mathcal{Y}}
\newcommand{\CZ}{\mathcal{Z}}

%
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cSO}{\mathcal{SO}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}


%
\newcommand{\BCA}{{\boldsymbol{\mathcal{A}}}}
\newcommand{\BCB}{{\boldsymbol{\mathcal{B}}}}
\newcommand{\BCC}{{\boldsymbol{\mathcal{C}}}}
\newcommand{\BCD}{{\boldsymbol{\mathcal{D}}}}
\newcommand{\BCE}{{\boldsymbol{\mathcal{E}}}}
\newcommand{\BCF}{{\boldsymbol{\mathcal{F}}}}
\newcommand{\BCG}{{\boldsymbol{\mathcal{G}}}}
\newcommand{\BCH}{{\boldsymbol{\mathcal{H}}}}
\newcommand{\BCI}{{\boldsymbol{\mathcal{I}}}}
\newcommand{\BCJ}{{\boldsymbol{\mathcal{J}}}}
\newcommand{\BCK}{{\boldsymbol{\mathcal{K}}}}
\newcommand{\BCL}{{\boldsymbol{\mathcal{L}}}}
\newcommand{\BCM}{{\boldsymbol{\mathcal{M}}}}
\newcommand{\BCN}{{\boldsymbol{\mathcal{N}}}}
\newcommand{\BCO}{{\boldsymbol{\mathcal{O}}}}
\newcommand{\BCP}{{\boldsymbol{\mathcal{P}}}}
\newcommand{\BCQ}{{\boldsymbol{\mathcal{Q}}}}
\newcommand{\BCR}{{\boldsymbol{\mathcal{R}}}}
\newcommand{\BCS}{{\boldsymbol{\mathcal{S}}}}
\newcommand{\BCT}{{\boldsymbol{\mathcal{T}}}}
\newcommand{\BCU}{{\boldsymbol{\mathcal{U}}}}
\newcommand{\BCV}{{\boldsymbol{\mathcal{V}}}}
\newcommand{\BCW}{{\boldsymbol{\mathcal{W}}}}
\newcommand{\BCX}{{\boldsymbol{\mathcal{X}}}}
\newcommand{\BCY}{{\boldsymbol{\mathcal{Y}}}}
\newcommand{\BCZ}{{\boldsymbol{\mathcal{Z}}}}

%
\newcommand{\FA}{\mathfrak{A}}
\newcommand{\FB}{\mathfrak{B}}
\newcommand{\FC}{\mathfrak{C}}
\newcommand{\FD}{\mathfrak{D}}
\newcommand{\FE}{\mathfrak{E}}
\newcommand{\FF}{\mathfrak{F}}
\newcommand{\FG}{\mathfrak{G}}
\newcommand{\FH}{\mathfrak{H}}
\newcommand{\FI}{\mathfrak{I}}
\newcommand{\FJ}{\mathfrak{J}}
\newcommand{\FK}{\mathfrak{K}}
\newcommand{\FL}{\mathfrak{L}}
\newcommand{\FM}{\mathfrak{M}}
\newcommand{\FN}{\mathfrak{N}}
\newcommand{\FO}{\mathfrak{O}}
\newcommand{\FP}{\mathfrak{P}}
\newcommand{\FQ}{\mathfrak{Q}}
\newcommand{\FR}{\mathfrak{R}}
\newcommand{\FS}{\mathfrak{S}}
\newcommand{\FT}{\mathfrak{T}}
\newcommand{\FU}{\mathfrak{U}}
\newcommand{\FV}{\mathfrak{V}}
\newcommand{\FW}{\mathfrak{W}}
\newcommand{\FX}{\mathfrak{X}}
\newcommand{\FY}{\mathfrak{Y}}
\newcommand{\FZ}{\mathfrak{Z}}

%
\newcommand{\Fa}{\mathfrak{a}}
\newcommand{\Fb}{\mathfrak{b}}
\newcommand{\Fc}{\mathfrak{c}}
\newcommand{\Fd}{\mathfrak{d}}
\newcommand{\Fe}{\mathfrak{e}}
\newcommand{\Ff}{\mathfrak{f}}
\newcommand{\Fg}{\mathfrak{g}}
\newcommand{\Fh}{\mathfrak{h}}
\newcommand{\Fi}{\mathfrak{i}}
\newcommand{\Fj}{\mathfrak{j}}
\newcommand{\Fk}{\mathfrak{k}}
\newcommand{\Fl}{\mathfrak{l}}
\newcommand{\Fm}{\mathfrak{m}}
\newcommand{\Fn}{\mathfrak{n}}
\newcommand{\Fo}{\mathfrak{o}}
\newcommand{\Fp}{\mathfrak{p}}
\newcommand{\Fq}{\mathfrak{q}}
\newcommand{\Fr}{\mathfrak{r}}
\newcommand{\Fs}{\mathfrak{s}}
\newcommand{\Ft}{\mathfrak{t}}
\newcommand{\Fu}{\mathfrak{u}}
\newcommand{\Fv}{\mathfrak{v}}
\newcommand{\Fw}{\mathfrak{w}}
\newcommand{\Fx}{\mathfrak{x}}
\newcommand{\Fy}{\mathfrak{y}}
\newcommand{\Fz}{\mathfrak{z}}

%
\newcommand{\BFA}{\boldsymbol{\mathfrak{A}}}
\newcommand{\BFB}{\boldsymbol{\mathfrak{B}}}
\newcommand{\BFC}{\boldsymbol{\mathfrak{C}}}
\newcommand{\BFD}{\boldsymbol{\mathfrak{D}}}
\newcommand{\BFE}{\boldsymbol{\mathfrak{E}}}
\newcommand{\BFF}{\boldsymbol{\mathfrak{F}}}
\newcommand{\BFG}{\boldsymbol{\mathfrak{G}}}
\newcommand{\BFH}{\boldsymbol{\mathfrak{H}}}
\newcommand{\BFI}{\boldsymbol{\mathfrak{I}}}
\newcommand{\BFJ}{\boldsymbol{\mathfrak{J}}}
\newcommand{\BFK}{\boldsymbol{\mathfrak{K}}}
\newcommand{\BFL}{\boldsymbol{\mathfrak{L}}}
\newcommand{\BFM}{\boldsymbol{\mathfrak{M}}}
\newcommand{\BFN}{\boldsymbol{\mathfrak{N}}}
\newcommand{\BFO}{\boldsymbol{\mathfrak{O}}}
\newcommand{\BFP}{\boldsymbol{\mathfrak{P}}}
\newcommand{\BFQ}{\boldsymbol{\mathfrak{Q}}}
\newcommand{\BFR}{\boldsymbol{\mathfrak{R}}}
\newcommand{\BFS}{\boldsymbol{\mathfrak{S}}}
\newcommand{\BFT}{\boldsymbol{\mathfrak{T}}}
\newcommand{\BFU}{\boldsymbol{\mathfrak{U}}}
\newcommand{\BFV}{\boldsymbol{\mathfrak{V}}}
\newcommand{\BFW}{\boldsymbol{\mathfrak{W}}}
\newcommand{\BFX}{\boldsymbol{\mathfrak{X}}}
\newcommand{\BFY}{\boldsymbol{\mathfrak{Y}}}
\newcommand{\BFZ}{\boldsymbol{\mathfrak{Z}}}

%
\newcommand{\BFa}{\boldsymbol{\mathfrak{a}}}
\newcommand{\BFb}{\boldsymbol{\mathfrak{b}}}
\newcommand{\BFc}{\boldsymbol{\mathfrak{c}}}
\newcommand{\BFd}{\boldsymbol{\mathfrak{d}}}
\newcommand{\BFe}{\boldsymbol{\mathfrak{e}}}
\newcommand{\BFf}{\boldsymbol{\mathfrak{f}}}
\newcommand{\BFg}{\boldsymbol{\mathfrak{g}}}
\newcommand{\BFh}{\boldsymbol{\mathfrak{h}}}
\newcommand{\BFi}{\boldsymbol{\mathfrak{i}}}
\newcommand{\BFj}{\boldsymbol{\mathfrak{j}}}
\newcommand{\BFk}{\boldsymbol{\mathfrak{k}}}
\newcommand{\BFl}{\boldsymbol{\mathfrak{l}}}
\newcommand{\BFm}{\boldsymbol{\mathfrak{m}}}
\newcommand{\BFn}{\boldsymbol{\mathfrak{n}}}
\newcommand{\BFo}{\boldsymbol{\mathfrak{o}}}
\newcommand{\BFp}{\boldsymbol{\mathfrak{p}}}
\newcommand{\BFq}{\boldsymbol{\mathfrak{q}}}
\newcommand{\BFr}{\boldsymbol{\mathfrak{r}}}
\newcommand{\BFs}{\boldsymbol{\mathfrak{s}}}
\newcommand{\BFt}{\boldsymbol{\mathfrak{t}}}
\newcommand{\BFu}{\boldsymbol{\mathfrak{u}}}
\newcommand{\BFv}{\boldsymbol{\mathfrak{v}}}
\newcommand{\BFw}{\boldsymbol{\mathfrak{w}}}
\newcommand{\BFx}{\boldsymbol{\mathfrak{x}}}
\newcommand{\BFy}{\boldsymbol{\mathfrak{y}}}
\newcommand{\BFz}{\boldsymbol{\mathfrak{z}}}

%
\newcommand{\DCA}{\mathscr{A}}
\newcommand{\DCB}{\mathscr{B}}
\newcommand{\DCC}{\mathscr{C}}
\newcommand{\DCD}{\mathscr{D}}
\newcommand{\DCE}{\mathscr{E}}
\newcommand{\DCF}{\mathscr{F}}
\newcommand{\DCG}{\mathscr{G}}
\newcommand{\DCH}{\mathscr{H}}
\newcommand{\DCI}{\mathscr{I}}
\newcommand{\DCJ}{\mathscr{J}}
\newcommand{\DCK}{\mathscr{K}}
\newcommand{\DCL}{\mathscr{L}}
\newcommand{\DCM}{\mathscr{M}}
\newcommand{\DCN}{\mathscr{N}}
\newcommand{\DCO}{\mathscr{O}}
\newcommand{\DCP}{\mathscr{P}}
\newcommand{\DCQ}{\mathscr{Q}}
\newcommand{\DCR}{\mathscr{R}}
\newcommand{\DCS}{\mathscr{S}}
\newcommand{\DCT}{\mathscr{T}}
\newcommand{\DCU}{\mathscr{U}}
\newcommand{\DCV}{\mathscr{V}}
\newcommand{\DCW}{\mathscr{W}}
\newcommand{\DCX}{\mathscr{X}}
\newcommand{\DCY}{\mathscr{Y}}
\newcommand{\DCZ}{\mathscr{Z}}

%
\newcommand{\BDCA}{{\boldsymbol{\mathscr{A}}}}
\newcommand{\BDCB}{{\boldsymbol{\mathscr{B}}}}
\newcommand{\BDCC}{{\boldsymbol{\mathscr{C}}}}
\newcommand{\BDCD}{{\boldsymbol{\mathscr{D}}}}
\newcommand{\BDCE}{{\boldsymbol{\mathscr{E}}}}
\newcommand{\BDCF}{{\boldsymbol{\mathscr{F}}}}
\newcommand{\BDCG}{{\boldsymbol{\mathscr{G}}}}
\newcommand{\BDCH}{{\boldsymbol{\mathscr{H}}}}
\newcommand{\BDCI}{{\boldsymbol{\mathscr{I}}}}
\newcommand{\BDCJ}{{\boldsymbol{\mathscr{J}}}}
\newcommand{\BDCK}{{\boldsymbol{\mathscr{K}}}}
\newcommand{\BDCL}{{\boldsymbol{\mathscr{L}}}}
\newcommand{\BDCM}{{\boldsymbol{\mathscr{M}}}}
\newcommand{\BDCN}{{\boldsymbol{\mathscr{N}}}}
\newcommand{\BDCO}{{\boldsymbol{\mathscr{O}}}}
\newcommand{\BDCP}{{\boldsymbol{\mathscr{P}}}}
\newcommand{\BDCQ}{{\boldsymbol{\mathscr{Q}}}}
\newcommand{\BDCR}{{\boldsymbol{\mathscr{R}}}}
\newcommand{\BDCS}{{\boldsymbol{\mathscr{S}}}}
\newcommand{\BDCT}{{\boldsymbol{\mathscr{T}}}}
\newcommand{\BDCU}{{\boldsymbol{\mathscr{U}}}}
\newcommand{\BDCV}{{\boldsymbol{\mathscr{V}}}}
\newcommand{\BDCW}{{\boldsymbol{\mathscr{W}}}}
\newcommand{\BDCX}{{\boldsymbol{\mathscr{X}}}}
\newcommand{\BDCY}{{\boldsymbol{\mathscr{Y}}}}
\newcommand{\BDCZ}{{\boldsymbol{\mathscr{Z}}}}

%
\newcommand{\SFA}{\mathsf{A}}
\newcommand{\SFB}{\mathsf{B}}
\newcommand{\SFC}{\mathsf{C}}
\newcommand{\SFD}{\mathsf{D}}
\newcommand{\SFE}{\mathsf{E}}
\newcommand{\SFF}{\mathsf{F}}
\newcommand{\SFG}{\mathsf{G}}
\newcommand{\SFH}{\mathsf{H}}
\newcommand{\SFI}{\mathsf{I}}
\newcommand{\SFJ}{\mathsf{J}}
\newcommand{\SFK}{\mathsf{K}}
\newcommand{\SFL}{\mathsf{L}}
\newcommand{\SFM}{\mathsf{M}}
\newcommand{\SFN}{\mathsf{N}}
\newcommand{\SFO}{\mathsf{O}}
\newcommand{\SFP}{\mathsf{P}}
\newcommand{\SFQ}{\mathsf{Q}}
\newcommand{\SFR}{\mathsf{R}}
\newcommand{\SFS}{\mathsf{S}}
\newcommand{\SFT}{\mathsf{T}}
\newcommand{\SFU}{\mathsf{U}}
\newcommand{\SFV}{\mathsf{V}}
\newcommand{\SFW}{\mathsf{W}}
\newcommand{\SFX}{\mathsf{X}}
\newcommand{\SFY}{\mathsf{Y}}
\newcommand{\SFZ}{\mathsf{Z}}

%
\newcommand{\SFa}{\mathsf{a}}
\newcommand{\SFb}{\mathsf{b}}
\newcommand{\SFc}{\mathsf{c}}
\newcommand{\SFd}{\mathsf{d}}
\newcommand{\SFe}{\mathsf{e}}
\newcommand{\SFf}{\mathsf{f}}
\newcommand{\SFg}{\mathsf{g}}
\newcommand{\SFh}{\mathsf{h}}
\newcommand{\SFi}{\mathsf{i}}
\newcommand{\SFj}{\mathsf{j}}
\newcommand{\SFk}{\mathsf{k}}
\newcommand{\SFl}{\mathsf{l}}
\newcommand{\SFm}{\mathsf{m}}
\newcommand{\SFn}{\mathsf{n}}
\newcommand{\SFo}{\mathsf{o}}
\newcommand{\SFp}{\mathsf{p}}
\newcommand{\SFq}{\mathsf{q}}
\newcommand{\SFr}{\mathsf{r}}
\newcommand{\SFs}{\mathsf{s}}
\newcommand{\SFt}{\mathsf{t}}
\newcommand{\SFu}{\mathsf{u}}
\newcommand{\SFv}{\mathsf{v}}
\newcommand{\SFw}{\mathsf{w}}
\newcommand{\SFx}{\mathsf{x}}
\newcommand{\SFy}{\mathsf{y}}
\newcommand{\SFz}{\mathsf{z}}

%
\newcommand{\TTA}{\mathtt{A}}
\newcommand{\TTB}{\mathtt{B}}
\newcommand{\TTC}{\mathtt{C}}
\newcommand{\TTD}{\mathtt{D}}
\newcommand{\TTE}{\mathtt{E}}
\newcommand{\TTF}{\mathtt{F}}
\newcommand{\TTG}{\mathtt{G}}
\newcommand{\TTH}{\mathtt{H}}
\newcommand{\TTI}{\mathtt{I}}
\newcommand{\TTJ}{\mathtt{J}}
\newcommand{\TTK}{\mathtt{K}}
\newcommand{\TTL}{\mathtt{L}}
\newcommand{\TTM}{\mathtt{M}}
\newcommand{\TTN}{\mathtt{N}}
\newcommand{\TTO}{\mathtt{O}}
\newcommand{\TTP}{\mathtt{P}}
\newcommand{\TTQ}{\mathtt{Q}}
\newcommand{\TTR}{\mathtt{R}}
\newcommand{\TTS}{\mathtt{S}}
\newcommand{\TTT}{\mathtt{T}}
\newcommand{\TTU}{\mathtt{U}}
\newcommand{\TTV}{\mathtt{V}}
\newcommand{\TTW}{\mathtt{W}}
\newcommand{\TTX}{\mathtt{X}}
\newcommand{\TTY}{\mathtt{Y}}
\newcommand{\TTZ}{\mathtt{Z}}

%
\newcommand{\TTa}{\mathtt{a}}
\newcommand{\TTb}{\mathtt{b}}
\newcommand{\TTc}{\mathtt{c}}
\newcommand{\TTd}{\mathtt{d}}
\newcommand{\TTe}{\mathtt{e}}
\newcommand{\TTf}{\mathtt{f}}
\newcommand{\TTg}{\mathtt{g}}
\newcommand{\TTh}{\mathtt{h}}
\newcommand{\TTi}{\mathtt{i}}
\newcommand{\TTj}{\mathtt{j}}
\newcommand{\TTk}{\mathtt{k}}
\newcommand{\TTl}{\mathtt{l}}
\newcommand{\TTm}{\mathtt{m}}
\newcommand{\TTn}{\mathtt{n}}
\newcommand{\TTo}{\mathtt{o}}
\newcommand{\TTp}{\mathtt{p}}
\newcommand{\TTq}{\mathtt{q}}
\newcommand{\TTr}{\mathtt{r}}
\newcommand{\TTs}{\mathtt{s}}
\newcommand{\TTt}{\mathtt{t}}
\newcommand{\TTu}{\mathtt{u}}
\newcommand{\TTv}{\mathtt{v}}
\newcommand{\TTw}{\mathtt{w}}
\newcommand{\TTx}{\mathtt{x}}
\newcommand{\TTy}{\mathtt{y}}
\newcommand{\TTz}{\mathtt{z}}

%
\newcommand{\Alpha}{\mathrm{A}}
\newcommand{\TBeta}{\mathrm{B}} %
\newcommand{\Epsilon}{\mathrm{E}}
\newcommand{\Zeta}{\mathrm{Z}}
\newcommand{\Eta}{\mathrm{H}}
\newcommand{\Iota}{\mathrm{I}}
\newcommand{\Kappa}{\mathrm{K}}
\newcommand{\Mu}{\mathrm{M}}
\newcommand{\Nu}{\mathrm{N}}
\newcommand{\Omikron}{\mathrm{O}}
\newcommand{\Rho}{\mathrm{P}}
\newcommand{\Tau}{\mathrm{T}}
\newcommand{\Chi}{\mathrm{X}}

%
\newcommand{\IAlpha}{A}
\newcommand{\IBeta}{B}
\newcommand{\IGamma}{\mathit{\Gamma}}
\newcommand{\IDelta}{\mathit{\Delta}}
\newcommand{\IEpsilon}{E}
\newcommand{\IZeta}{Z}
\newcommand{\IEta}{H}
\newcommand{\ITheta}{\mathit{\Theta}}
\newcommand{\IIota}{I}
\newcommand{\IKappa}{K}
\newcommand{\ILambda}{\mathit{\Lambda}}
\newcommand{\IMu}{M}
\newcommand{\INu}{N}
\newcommand{\IXi}{\mathit{\Xi}}
\newcommand{\IOmikron}{O}
\newcommand{\IPi}{\mathit{\Pi}}
\newcommand{\IRho}{P}
\newcommand{\ISigma}{\mathit{\Sigma}}
\newcommand{\ITau}{T}
\newcommand{\IUpsilon}{\mathit{\Upsilon}}
\newcommand{\IPhi}{\mathit{\Phi}}
\newcommand{\IChi}{X}
\newcommand{\IPsi}{\mathit{\Psi}}
\newcommand{\IOmega}{\mathit{\Omega}}

%
\newcommand{\omikron}{o}

%
\newcommand{\BAlpha}{{\boldsymbol{\Alpha}}}
\newcommand{\BBeta}{{\boldsymbol{\Beta}}}
\newcommand{\BGamma}{{\boldsymbol{\Gamma}}}
\newcommand{\BDelta}{{\boldsymbol{\Delta}}}
\newcommand{\BEpsilon}{{\boldsymbol{\Epsilon}}}
\newcommand{\BZeta}{{\boldsymbol{\Zeta}}}
\newcommand{\BEta}{{\boldsymbol{\Eta}}}
\newcommand{\BTheta}{{\boldsymbol{\Theta}}}
\newcommand{\BIota}{{\boldsymbol{\Iota}}}
\newcommand{\BKappa}{{\boldsymbol{\Kappa}}}
\newcommand{\BLambda}{{\boldsymbol{\Lambda}}}
\newcommand{\BMu}{{\boldsymbol{\Mu}}}
\newcommand{\BNu}{{\boldsymbol{\Nu}}}
\newcommand{\BXi}{{\boldsymbol{\Xi}}}
\newcommand{\BOmikron}{{\boldsymbol{\Omikron}}}
\newcommand{\BPi}{{\boldsymbol{\Pi}}}
\newcommand{\BRho}{{\boldsymbol{\Rho}}}
\newcommand{\BSigma}{{\boldsymbol{\Sigma}}}
\newcommand{\BTau}{{\boldsymbol{\Tau}}}
\newcommand{\BUpsilon}{{\boldsymbol{\Upsilon}}}
\newcommand{\BPhi}{{\boldsymbol{\Phi}}}
\newcommand{\BChi}{{\boldsymbol{\Chi}}}
\newcommand{\BPsi}{{\boldsymbol{\Psi}}}
\newcommand{\BOmega}{{\boldsymbol{\Omega}}}

%
\newcommand{\BIAlpha}{{\boldsymbol{\IAlpha}}}
\newcommand{\BIBeta}{{\boldsymbol{\IBeta}}}
\newcommand{\BIGamma}{{\boldsymbol{\IGamma}}}
\newcommand{\BIDelta}{{\boldsymbol{\IDelta}}}
\newcommand{\BIEpsilon}{{\boldsymbol{\IEpsilon}}}
\newcommand{\BIZeta}{{\boldsymbol{\IZeta}}}
\newcommand{\BIEta}{{\boldsymbol{\IEta}}}
\newcommand{\BITheta}{{\boldsymbol{\ITheta}}}
\newcommand{\BIIota}{{\boldsymbol{\IIota}}}
\newcommand{\BIKappa}{{\boldsymbol{\IKappa}}}
\newcommand{\BILambda}{{\boldsymbol{\ILambda}}}
\newcommand{\BIMu}{{\boldsymbol{\IMu}}}
\newcommand{\BINu}{{\boldsymbol{\INu}}}
\newcommand{\BIXi}{{\boldsymbol{\IXi}}}
\newcommand{\BIOmikron}{{\boldsymbol{\IOmikron}}}
\newcommand{\BIPi}{{\boldsymbol{\IPi}}}
\newcommand{\BIRho}{{\boldsymbol{\IRho}}}
\newcommand{\BISigma}{{\boldsymbol{\ISigma}}}
\newcommand{\BITau}{{\boldsymbol{\ITau}}}
\newcommand{\BIUpsilon}{{\boldsymbol{\IUpsilon}}}
\newcommand{\BIPhi}{{\boldsymbol{\IPhi}}}
\newcommand{\BIChi}{{\boldsymbol{\IChi}}}
\newcommand{\BIPsi}{{\boldsymbol{\IPsi}}}
\newcommand{\BIOmega}{{\boldsymbol{\IOmega}}}

%
\newcommand{\Balpha}{{\boldsymbol{\alpha}}}
\newcommand{\Bbeta}{{\boldsymbol{\beta}}}
\newcommand{\Bgamma}{{\boldsymbol{\gamma}}}
\newcommand{\Bdelta}{{\boldsymbol{\delta}}}
\newcommand{\Bepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\Bzeta}{{\boldsymbol{\zeta}}}
\newcommand{\Beta}{{\boldsymbol{\eta}}}
\newcommand{\Btheta}{{\boldsymbol{\theta}}}
\newcommand{\Biota}{{\boldsymbol{\iota}}}
\newcommand{\Bkappa}{{\boldsymbol{\kappa}}}
\newcommand{\Blambda}{{\boldsymbol{\lambda}}}
\newcommand{\Bmu}{{\boldsymbol{\mu}}}
\newcommand{\Bnu}{{\boldsymbol{\nu}}}
\newcommand{\Bxi}{{\boldsymbol{\xi}}}
\newcommand{\Bomikron}{{\boldsymbol{\omikron}}}
\newcommand{\Bpi}{{\boldsymbol{\pi}}}
\newcommand{\Brho}{{\boldsymbol{\rho}}}
\newcommand{\Bsigma}{{\boldsymbol{\sigma}}}
\newcommand{\Btau}{{\boldsymbol{\tau}}}
\newcommand{\Bupsilon}{{\boldsymbol{\upsilon}}}
\newcommand{\Bphi}{{\boldsymbol{\phi}}}
\newcommand{\Bchi}{{\boldsymbol{\chi}}}
\newcommand{\Bpsi}{{\boldsymbol{\psi}}}
\newcommand{\Bomega}{{\boldsymbol{\omega}}}
\newcommand{\Bvarepsilon}{{\boldsymbol{\varepsilon}}}
\newcommand{\Bvarphi}{{\boldsymbol{\varphi}}}
\newcommand{\Bvarpi}{{\boldsymbol{\varpi}}}
\newcommand{\Bvarrho}{{\boldsymbol{\varrho}}}
\newcommand{\Bvarsigma}{{\boldsymbol{\varsigma}}}
\newcommand{\Bvartheta}{{\boldsymbol{\vartheta}}}




\newcommand{\DD}{\mathbb{D}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\JJ}{\mathbb{J}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\OO}{\mathbb{O}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\UU}{\mathbb{U}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\WW}{\mathbb{W}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}}


\newcommand{\rmp}{\textrm{p}}
\newcommand{\pa}{\textrm{pa}}
\newcommand{\ch}{\textrm{ch}}
\newcommand{\ancs}{\textrm{ancs}}
\newcommand{\desc}{\textrm{desc}}
\newcommand{\rmg}{\textrm{g}}
\newcommand{\rmq}{\textrm{q}}
\newcommand{\rmm}{\textrm{m}}
\newcommand{\g}{\, | \,}
\newcommand{\bA}{\bm{A}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bX}{\bm{X}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\s}{\, ; \,}
\newcommand{\iid}{\stackrel{iid}{\sim}}

%
\newcommand{\NORMAL}{\CN} %
\newcommand{\MVNORMAL}{\CM\CV\CN} %
\newcommand{\GP}{\mathcal{GP}} %
\newcommand{\R}{\mathbb{R}} %
\newcommand{\Q}{\mathbb{Q}} %
\newcommand{\Z}{\mathbb{Z}} %
\newcommand{\N}{\mathbb{N}} %
\newcommand{\T}{\mathbb{T}} %
\newcommand{\C}{\mathbb{C}} %
\newcommand{\B}{\mathbb{B}}
\newcommand{\vecone}{\mathbf{1}} %
\newcommand{\veczero}{\mathbf{0}} %
\newcommand{\vecinfty}{\boldsymbol{\infty}} %
\newcommand{\TRANSP}{\mathsf{T}} %
\newcommand{\DIFF}{\Td} %
\newcommand{\DIFFX}[1]{\,\Td{#1}} %
\newcommand{\DIFFM}[2]{\,{#1}\!\left({#2}\right)} %
\newcommand{\lspan}{\overline{\mathrm{span}}} %
\newcommand{\diag}{\mathrm{diag}} %
\newcommand{\logistic}{\mathrm{logistic}} %
\newcommand{\logit}{\mathrm{logit}} %
\newcommand{\PROB}{\mathbb{P}} %
\newcommand{\PR}{\mathrm{Pr}} %
\newcommand{\EXP}{\mathbb{E}} %
\newcommand{\VAR}{\mathrm{Var}} %
\newcommand{\COV}{\mathrm{Cov}} %
\newcommand{\CORR}{\mathrm{Corr}} %
\newcommand{\MOD}{\mathrm{mod}} %
\newcommand{\realpart}{\mathrm{Re}} %
\newcommand{\imagpart}{\mathrm{Im}} %
\newcommand{\clos}{\mathrm{cl}} %
\newcommand{\inter}[1]{\mathrm{int}(#1)} %
\newcommand{\relint}{\mathrm{relint}} %
\newcommand{\relbd}{\mathrm{relbd}} %
\newcommand{\supp}{\mathrm{supp}} %
\newcommand{\conv}{\mathrm{conv}} %
\newcommand{\aff}{\mathrm{aff}} %
\newcommand{\cone}{\mathrm{cone}} %
\newcommand{\dual}{\mathrm{dual}} %
\newcommand{\dom}{\mathrm{dom}} %
\newcommand{\epigraph}{\mathrm{epi}} %
\newcommand{\tr}{\mathrm{tr}} %
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\diver}[1]{\,\mathrm{div}(#1)}
%
\newcommand{\Id}{\mathrm{Id}}
\newcommand{\range}{\mathrm{Range}}
\newcommand{\Unif}{\mathrm{Unif}}
\newcommand{\vae}{\varepsilon}
\newcommand{\density}[2]{\frac{d#1}{d#2}}
\newcommand{\logden}[2]{\log\left(frac{d#1}{d#2}\right)}
%
\newcommand{\rom}[1]{%
  \textup{\uppercase\expandafter{\romannumeral#1}}%
}
\newcommand{\law}{\mathrm{Law}}
\newcommand{\inner}[2]{\langle #1,#2\rangle}
\newcommand{\coker}[1]{\text{coker}(#1)}
\newcommand{\kernel}[1]{\text{ker}(#1)}
\newcommand{\im}[1]{\text{im}(#1)}
\newcommand{\ix}[1]{\text{index}(#1)}
\newcommand{\spt}{\text{spt}}
\newcommand{\Tan}{\mathrm{Tan}}
\newcommand{\QV}[1]{\langle #1\rangle}
\newcommand{\qqquad}{\quad\quad\quad}
%

%
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\purple}[1]{\textcolor{purple}{#1}}


%
\DeclareMathOperator*{\argmin}{arg\,min} %
\DeclareMathOperator*{\argmax}{arg\,max} %
\DeclareMathOperator*{\minimize}{\mathrm{minimize}} %
\DeclareMathOperator*{\maximize}{\mathrm{maximize}} %


%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}


\newcommand{\Hnull}{\mathcal{H}_0}
\newcommand{\Halt}{\mathcal{H}_1}
\newcommand{\TODO}[1]{\textcolor{red}{#1}}

%
\newcommand{\ssubset}{\subset\joinrel\subset}

%

%
\newcommand{\kl}[2]{H\left( #1 \mid #2\right)}
\newcommand{\E}{\mathbb{E}}
\def \d {\rm d}



\newcommand{\proj}{\text{proj}}
%

\newcommand*{\Var}{\mathbb Var}
%
\newcommand*{\pp}[2]{\mathbb P_{#1}\left\{#2\right\}}
\DeclareMathOperator{\var}{Var}
\DeclareMathOperator{\cov}{Cov}
\newcommand*{\indic}[1]{\mathbf{1}_{\left\{#1\right\}}}
\newcommand*{\ep}{\varepsilon}
\newcommand*{\defeq}{\coloneqq}
\newcommand*{\rd}{\mathrm{d}}
\newcommand*{\dd}{\, \rd}
\newcommand{\D}{\mathrm d}

\newcommand{\bbT}{\mathbb T}

\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\cleq}{\,\preceq_{\rm c}\,}
\DeclareMathOperator{\ncleq}{\,\not\preceq_{\rm c}\,}
\DeclareMathOperator{\vsubseteq}{\mathrel{\rotatebox{-90}{$\subseteq$}}}


%
%
